Smoothed Analysis of the k-Swap Neighborhood for Makespan Scheduling

Local search is a widely used technique for tackling challenging optimization problems, offering simplicity and strong empirical performance across various problem domains. In this paper, we address the problem of scheduling a set of jobs on identical parallel machines with the objective of makespan minimization, by considering a local search neighborhood, called $k$-swap. A $k$-swap neighbor is obtained by interchanging the machine allocations of at most $k$ jobs scheduled on two machines. While local search algorithms often perform well in practice, they can exhibit poor worst-case performance. In our previous study, we showed that for $k \geq 3$, there exists an instance where the number of iterations required to converge to a local optimum is exponential in the number of jobs. Motivated by this discrepancy between theoretical worst-case bound and practical performance, we apply smoothed analysis to the $k$-swap local search. Smoothed analysis has emerged as a powerful framework for analyzing the behavior of algorithms, aiming to bridge the gap between poor worst-case and good empirical performance. In this paper, we show that the smoothed number of iterations required to find a local optimum with respect to the $k$-swap neighborhood is bounded by $O(m^2 \cdot n^{2k+2} \cdot \log m \cdot \phi)$, where $n$ and $m$ are the numbers of jobs and machines, respectively, and $\phi \geq 1$ is the perturbation parameter. The bound on the smoothed number of iterations demonstrates that the proposed lower bound reflects a pessimistic scenario which is rare in practice.

==> content/Conclusion.tex <==
\section{Concluding Remarks}



==> content/WorstCase.tex <==
\section{Worst-case Analysis}
In this part, we analyze the number of iterations required in the worst case to find a swap-optimal solution.
First of all, according to a result by Frank and Tardos~\cite{frank1987application}, we show that we can assume w.l.o.g. that all the processing times of the jobs are integers and are bounded by $O(2^{O(n^3)})$. Frank and Tardos provided an algorithm which takes a rational vector $W = (w_1, ... , w_n)$ and an integer $N$ and outputs an integral vector $W' = (w'_1, ... , w'_n)$ such that $\lVert W' \rVert_\infty \leq 2^{4n^3} N^{n(n+2)}$ and sign $(W \cdot b)$ = sign $(W' \cdot b)$ whenever $b$ is an integer vector with $\lVert b \rVert_1 \leq N - 1$ (sign$(x)$ is the signum function that returns +1, -1 or 0). In our problem, let $P = (p_1, ..., p_n)$ be a rational vector of the processing times, $N = n + 3$, and $P' = (p'_1, ..., p'_n)$ be an integral vector such that $\lVert P' \rVert_\infty \leq O(2^{O(n^3)})$. If we want to consider integral processing times which are upper-bounded by $O(2^{O(n^3)})$ as the input of our problem, we need to show that for all the critical machines $i$ and non-critical machines $i'$, and for all $j \in M_i$ and $j' \in M_{i'}$, we have $0 < p_j - p_{j'} < L_i - L_{i'}$ \textit{iff}  $0 < p'_j -  p'_{j'} < L'_i - L'_{i'}$, where $L_i$ and $L_{i'}$ are the loads of machines $i$ and $i'$ with respect to the vector $P$, respectively, and $L'_i$ and $L'_{i'}$ are the loads of machines $i$ and $i'$ with respect to the vector $P'$, respectively. More clearly, when we have a sequence of improving swaps with the processing times in vector $P$, we should also have the same sequence with the processing times in vector $P'$. 

\begin{lemma}
    \label{lem:boundPs}
    In the problem $P||C_{max}$, if we consider a vector $P'$ of processing times instead of $P$, such that $\lVert P' \rVert_\infty \leq O(2^{O(n^3)})$, the sequence of improving swaps in obtaining a swap-optimal solution stays the same.
\end{lemma}
\begin{proof}
First, we show that $p_j - p_{j'} > 0$ \textit{iff}  $p'_j -  p'_{j'} > 0$ (for all $j \neq j' \in \{ 1, ... , n \}$). 
To this end, we consider a vector $b = e_j - e_{j'}$, such that $e_j$ is an $n$-dimensional vector with $(e_j)_j = 1$ and $(e_j)_x = 0$, for all $x \neq j$. We have $\lVert b \rVert_1 = 2 \leq n + 2$. Also, we have $P \cdot b = p_j - p_{j'} > 0$. Since sign($P \cdot b$) = sign($P' \cdot b$), we have $P' \cdot b = p'_j - p'_{j'} > 0$. 
Next, we show that for all the critical machines $i$ and non-critical machines $i'$, and for all $j \in M_i$ and $j' \in M_{i'}$, we have $p_j - p_{j'} < L_i - L_{i'}$ \textit{iff}  $p'_j -  p'_{j'} < L'_i - L'_{i'} $.
Here, we consider a vector $b = e_j - e_{j'} - \sum_{j'' \in M_i} e_{j''} + \sum_{j''' \in M_{i'}} e_{j'''}$. We have $\lVert b \rVert_1 \leq n + 2$. Also, we have $P \cdot b = p_j - p_{j'} - (L_i - L_{i'}) < 0$. Since sign($P \cdot b$) = sign($P' \cdot b$), we have $P' \cdot b = p'_j - p'_{j'} - (L'_i - L'_{i'}) < 0$.
\end{proof}

For counting the number of improving swaps in obtaining a swap optimal solution, we divide them into different phases of improvement. Each phase $h$ contains $\lambda_h$ improving swaps ($\lambda_h \geq 0$). Let $\Delta_h$ be the value of $\Delta$ at the beginning of phase $h$. In every iteration $t$ of phase $h$, we have $\frac{\Delta_h}{2} < \Delta(t) \leq \Delta_h$. More precisely, we start phase $h+1$ as soon as we get $\Delta \leq \frac{\Delta_h}{2}$. Since all the processing times of the jobs are integral, they are bounded by $O(2^{O(n^3)})$, and we have $\Delta_{h+1} \leq \frac{\Delta_h}{2}$ (due to the monotonicity of the values of $\Delta$), the total number of phases is upper-bounded by $O(n^3)$. Therefore, we only need to analyze the number of improving swaps in each phase $h$, for $0 \leq h \leq O(n^3)$.

For analyzing the number of improving swaps in phase $h$, we split the set of machines in our schedule at the start of iteration $t$ into two sets $\gamma_l^t = \{ i: L_i(t) \geq L_{max}(t) - \frac{\Delta_h}{2} \}$ and $\gamma_s^t = \{ i: L_i(t) < L_{max}(t) - \frac{\Delta_h}{2} \}$.
We have $|\gamma_l^t| > 0$ since the set of critical machines is always in $\gamma_l^t$. We also have $|\gamma_s^t| > 0$  since we have $\frac{\Delta_h}{2} < \Delta(t)$.
With a slight abuse of notation, we refer to these two sets as $\gamma_l$ and $\gamma_s$.
We show that the values of $|\gamma_l|$ are non-decreasing.

\begin{lemma}
\label{lem:gammalNonDec}
In a phase $h$ of obtaining a swap-optimal solution, the values of $|\gamma_l|$ are non-decreasing.
\end{lemma}
\begin{proof}
    In every iteration, we swap a job $j \in M_i$ with a job $j' \in M_{i'}$ such that $i$ and $i'$ are critical and non-critical machines, respectively. Since we have $p_j > p_{j'}$, $L_i$ decreases and $L_{i'}$ increases. As the values of $L_{\max}(t) - \frac{\Delta_h}{2}$ are non-increasing (in every iteration, either $L_{\max}$ stays the same or decreases) and only $L_i$ decreases, no machine $i'' \neq i$ in the set $\gamma_l$ moves to the set $\gamma_s$. So, the only machine that can move to the set $\gamma_s$ is machine $i$. We show that if $i$ moves to $\gamma_s$, then $i'$ moves to $\gamma_l$. If after swapping $j \in M_i$ with $j' \in M_{i'}$ in iteration $t$, machine $i$ moves to $\gamma_s$, we get:
    \begin{align*}
        L_{i}(t+1) < L_{\max}(t+1) - \frac{\Delta_h}{2}
        &\phantom{}\Rightarrow L_{i}(t) - L_{i}(t+1) > L_{i}(t) - (L_{\max}(t+1) - \frac{\Delta_h}{2}) \\
        &\Rightarrow p_j - p_{j'} > L_{i}(t) - (L_{\max}(t+1) - \frac{\Delta_h}{2}).
    \end{align*}
    According to the above inequality, and since machine $i$ is a critical machine at the start of iteration $t$, we get the following:
    \begin{align*}
        L_{i'}(t+1) = L_{i'}(t) + p_j - p_{j'}
        &\phantom{}> L_{i'}(t) + L_{i}(t) - (L_{\max}(t+1) - \frac{\Delta_h}{2}) \\
        &= L_{i'}(t) + L_{\max}(t) - L_{\max}(t+1) + \frac{\Delta_h}{2} \\
        &\geq  L_{i'}(t) + L_{\max}(t+1) - L_{\max}(t+1) + \frac{\Delta_h}{2} \\
        &=  L_{i'}(t) + \frac{\Delta_h}{2} \geq L_{\min}(t) + \frac{\Delta_h}{2}.
    \end{align*} As the values of $\Delta$ are non-increasing, we have
    \begin{align*}
        \Delta(t) \leq \Delta_h
        &\phantom{}\Rightarrow L_{\max}(t) - L_{\min}(t) \leq \Delta_h \\
        &\Rightarrow L_{\max}(t) - \frac{\Delta_h}{2} \leq L_{\min}(t) + \frac{\Delta_h}{2}.
    \end{align*}
    Therefore, we get 
    \begin{align*}
        L_{i'}(t+1) \geq L_{\min}(t) + \frac{\Delta_h}{2} \geq L_{\max}(t) - \frac{\Delta_h}{2} \geq L_{\max}(t+1) - \frac{\Delta_h}{2}.
    \end{align*}
    So, we got $L_{i'}(t+1) >  L_{\max}(t+1) - \frac{\Delta_h}{2}$, which means that if $i$ moves to $\gamma_s$, $i'$ moves to $\gamma_l$. Thus, the values of $|\gamma_l|$ are non-decreasing.
\end{proof}

%As a result of the lemma~\ref{lem:gammalNonDec}, we have the following corollary. 

%\begin{corollary}
%\label{cor:moveToGammaL}
%If we swap two jobs between a critical machine $i \in \gamma_l$ and a non-critical %machine $i' \in \gamma_s$, and $i$ moves to $\gamma_s$, then $i'$ moves to $\gamma_l$.
%\end{corollary}

As all the critical machines are in the set $\gamma_l$, we either swap two jobs inside the set $\gamma_l$ or we swap two jobs between a critical machine $i \in \gamma_l$ and a non-critical machine $i' \in \gamma_s$. In neither of the cases, the loads of the machines in the set $\gamma_s$ decreases (Note that according to Lemma~\ref{lem:gammalNonDec}, if we swap two jobs between a critical machine $i \in \gamma_l$ and a non-critical machine $i' \in \gamma_s$, and $i$ moves to $\gamma_s$, then $i'$ moves to $\gamma_l$). Consequently, we have the following corollary.

\begin{corollary}
\label{cor:lMaxMinusLlMin}
For all the $\ell$min-load machines in the set $\gamma_s$, the values of $L_{\ell\min}$ are non-decreasing in phase $h$ of obtaining a swap-optimal solution.
\end{corollary}

Next, we proceed with establishing an upper bound for the number of improving swaps in order to obtain a swap-optimal solution. To this end, we first provide the following lemmas and corollaries.

\begin{lemma}
    \label{lem:remainLMinLoad}
    A non-critical machine $i$ remains non-critical for at most $O(n^2)$ iterations in which we do swaps between $i$ and critical machines.
\end{lemma}

\begin{proof}
    Let $J = \{j_1, j_2, \dotsc, j_n\}$ be the set of jobs in $\sigma$ such that $p_{j_n} \geq p_{j_{n-1}} \geq \dotsc \geq p_{j_1}$. For $k \in \{1, 2, \dotsc, n\}$, we define $\mathrm{rank}(j_k) = k$.
    We define $\Phi = \sum_{k: j_k \in M_i} \mathrm{rank}(j_k)$. We have $1 \leq \Phi \leq n^2$.
    In every iteration where we swap a job $j \in M_i$ with a job $j' \in M_{i'}$ such that $i'$ is a critical machine, the value of $\Phi$ increases at least by one as we have $p_j < p_{j'}$.
\end{proof}

\begin{lemma}
    \label{lem:fixTwojobs}
    Let $i \in \gamma_l$ and $i' \in \gamma_s$ be the critical and $\ell$min-load machines in iteration $t$ of phase $h$, respectively, and for jobs $j \in M_i$ and $j' \in M_{i'}$, we have $0 < p_j - p_{j'} < L_{\max}(t) - L_{\ell\min}(t)$. If after swapping jobs $j$ and $j'$ in iteration $t$, machine $i'$ becomes a critical load machine, we are not able to swap the jobs $j$ and $j'$ with each other on a critical and an $\ell$min-load machine in the remaining iterations of phase $h$.
\end{lemma}

\begin{proof}
    After swapping jobs $j$ and $j'$ with each other in iteration $t$, we get:
    \begin{align*}
        L_{\max}(t+1) - L_{\ell\min}(t+1)
        &\phantom{}= L_{i'}(t+1) - L_{\ell\min}(t+1) \\
        &= L_{i'}(t) + p_j - p_{j'} - L_{\ell\min}(t+1) \\
        &\leq L_{i'}(t) + p_j - p_{j'} - L_{\ell\min}(t) \\
        &= L_{i'}(t) + p_j - p_{j'} - L_{i'}(t) = p_j - p_{j'}.
    \end{align*}
    Since the values of $L_{\max} - L_{\ell\min}$ are non-increasing (according to corollary~\ref{cor:lMaxMinusLlMin}), we are not able to swap job $j$ with job $j'$ on a critical machine and an $\ell$min-load machine in all the remaining iterations of phase $h$.
\end{proof}

According to Lemma~\ref{lem:fixTwojobs}, if after swapping a job $j$ on a critical machine $i$ with a job $j'$ on a non-critcical machine $i' \in \gamma_s$, $i'$ becomes a critical machine, we are not able to swap $j$ with $j'$ on a critical machine and an $\ell$min-load machine in all the remaining iteration of phase $h$ anymore. However, it might be possible to swap these two jobs on a critical machine and an $\ell'$min-load machine, for an $\ell' < \ell$. Since we have $O(m)$ machines with a load less than $L_{\ell\min}$, we have at most $O(m \cdot n^2)$ swaps, which cause a non-critical machine $i' \in \gamma_s$ to become a critical machine.

\begin{corollary}
\label{cor:NumberOftimesToMoveToGammaS}
A non-critical machine $i \in \gamma_s$ becomes critical for at most $O(m \cdot n^2)$ times.
\end{corollary}

\begin{theorem}
    \label{thm:numberOf2Swaps}
    The number of improving swaps in phase $h$ of obtaining a swap optimal solution is upper-bounded by $O(n^2 \cdot (m^3 \cdot n^4)^{m-2}) = O(m^{3m - 6} \cdot n^{4m - 6})$.
\end{theorem}

\begin{proof}
    We do the proof based on induction on the number of machines. For the base case, we have $m=1$, and we are not able to do any swaps. Now, suppose that the theorem holds for $m-1$ machines. We will show that it also holds for $m$ machines. 
    In the set $\gamma_l$, we have at most $m-1$ machines (since $|\gamma_s| > 0$). Therefore, according to the induction hypothesis, we have at most $O(n^2 \cdot (m^3 \cdot n^4)^{m-3})$ consecutive swaps among the machines in the set $\gamma_l$ (We refer to these kinds of swaps as \emph{type 1} swaps). 
    Based on Corollary~\ref{cor:NumberOftimesToMoveToGammaS}, we have at most $O(m^2 \cdot n^2)$ swaps between the machines in $\gamma_l$ and $\gamma_s$ such that a non-critical machine in the set $\gamma_s$ becomes critical (We refer to these kinds of swaps as \emph{type 2} swaps). According to Lemma~\ref{lem:remainLMinLoad}, between any two consecutive swaps of type 2, we have at most $O(m \cdot n^2)$ consecutive swaps between the machines in $\gamma_l$ and $\gamma_s$ when none of the non-critical machines in the set $\gamma_s$ becomes critical (We refer to these kinds of swaps as \emph{type 3} swaps). Furthermore, according to the induction hypothesis, and since the swaps between the critical machines in $\gamma_l$ do not change the non-critical machine in $\gamma_s$, we have at most $O(n^2 \cdot (m^3 \cdot n^4)^{m-3})$ consecutive swaps of type 1 between any two swaps of type 3.
    Hence, in total, we have $O(n^2 \cdot (m^3 \cdot n^4)^{m-3} \cdot m^3 \cdot n^4) = O(n^2 \cdot (m^3 \cdot n^4)^{m-2})$ swaps.
\end{proof}

According to Theorem~\ref{thm:numberOf2Swaps}, we have at most $O(m^{3m -6} \cdot n^{4m - 6})$ improving swaps in phase $h$, and the total number of phases is upper-bounded by $O(n^3)$. Thus, we have the following corollary.

\begin{corollary}
    \label{cor:totalNumberOfSwaps}
    The total number of improving swaps in obtaining a swap-optimal solution for the problem $P||C_{max}$ is upper-bounded by $O(m^{3m -6} \cdot n^{4m - 3})$.
\end{corollary}

According to Corollary~\ref{cor:totalNumberOfSwaps}, the total number of improving swaps in obtaining a swap optimal solution is upper-bounded by $O(m^{3m -6} \cdot n^{4m - 3})$. Since a swap neighborhood contains all the possible jumps and swaps, we should also count the number of jumps in obtaining a swap optimal solution.
To do so, we count the number of jumps similar to Brucker et al.~\cite{brucker1997improving}, who provided an upper bound on the number of jumps in converging to a local optimum for the problem $P||C_{\max}$.

\begin{theorem}
\label{thrm:2-swapOptSol}
The total number of improving iterations in finding a swap optimal solution is upper-bounded by $O(m^{3m -6} \cdot n^{4m - 1})$.
\end{theorem}

\begin{proof}
    Let $j$ be a job that jumps to the machine $i$ in iteration $t$, and after this iteration, machine $i$ becomes a critical machine. Assume w.l.o.g. that machine $i$ is a min-load machine at the start of iteration $t$. After the jump, we get:
    \begin{align*}
        \Delta(t+1)
        = L_{i}(t+1) - L_{\min}(t+1)
        = L_{i}(t) + p_j - L_{\min}(t+1)
        &\phantom{}\leq L_{i}(t) + p_j - L_{\min}(t)\\
        &= L_{i}(t) + p_j - L_{i}(t) = p_j.
    \end{align*}
    As the values of $\Delta$ in obtaining a swap optimal solution are non-increasing, job $j$ cannot be jumped for the second time.
    Therefore, in at most $O(n)$ iterations, the critical machine changes by performing a jump operator.
    Between two consecutive jumps such that the critical machine changes, we have at most $O(m^{3m -6} \cdot n^{4m - 3})$ swaps according to Corollary~\ref{cor:totalNumberOfSwaps}. 
    Also, between two consecutive swaps, we can have at most $O(n)$ jumps such that the set of critical machines remains the same. Note that if by performing a jump operator the set of critical machines remains the same, the number of swaps does not increase by more than one as the load of none of the machines in the schedule decreases.
    Thus, the total number of improving iterations is upper-bounded by $O(m^{3m -6} \cdot n^{4m - 1})$.
\end{proof}

